SSR: Spatial Sequential Hybrid Architecture for Latency Throughput Tradeoff in Transformer Acceleration

With the increase in the computation intensity of the chip, the mismatch between computation layer shapes and the available computation resource significantly limits the utilization of the chip. Driven by this observation, prior works discuss spatial accelerators or dataflow architecture to maximize the throughput. However, using spatial accelerators could potentially increase the execution latency. In this work, we first systematically investigate two execution models: (1) sequentially (temporally) launch one monolithic accelerator, and (2) spatially launch multiple accelerators. From the observations, we find that there is a latency throughput tradeoff between these two execution models, and combining these two strategies together can give us a more efficient latency throughput Pareto front. To achieve this, we propose spatial sequential architecture (SSR) and SSR design automation framework to explore both strategies together when deploying deep learning inference. We use the 7nm AMD Versal ACAP VCK190 board to implement SSR accelerators for four end-to-end transformer-based deep learning models. SSR achieves average throughput gains of 2.53x, 35.71x, and 14.20x under different batch sizes compared to the 8nm Nvidia GPU A10G, 16nm AMD FPGAs ZCU102, and U250. The average energy efficiency gains are 8.51x, 6.75x, and 21.22x, respectively. Compared with the sequential-only solution and spatial-only solution on VCK190, our spatial-sequential-hybrid solutions achieve higher throughput under the same latency requirement and lower latency under the same throughput requirement. We also use SSR analytical models to demonstrate how to use SSR to optimize solutions on other computing platforms, e.g., 14nm Intel Stratix 10 NX.

==> 5_SSR_DSE.tex <==

\section{SSR Framework and Design Space Exploration}
\label{sec:DSE}


% last subsection in framework section
\subsection{Automatic Source Code Generation and Compilation}
\label{sec:acg}
Our ~\M~ framework includes a Python-based code generation toolflow. 
Based on our analytical model guided design space exploration, the code generation toolflow can instantiate the code template to generate the design source code files including ARM CPU host code, FPGA high-level synthesis code, and AIE intrinsic C/C++ code.
Then ~\M~ framework then calls corresponding backend tools in AMD Vitis~\cite{vitis} to generate both the hardware bitstream and host binaries, which can be readily deployed on the board.


==> Listing_Dataflow.tex <==
% \vspace{-10pt}
% \begin{figure}[t]
% https://tex.stackexchange.com/questions/62720/vertical-space-after-algorithm
\setlength{\textfloatsep}{0pt}% Remove \textfloatsep
\begin{algorithm}
% \begin{minipage}{\columnwidth-8pt}
\caption{Dataflow of a Spatial Accelerator}
\begin{minted}[fontsize=\footnotesize, linenos]{c}
// PL On-chip Buffer Reuse Time Loop
for(int bat=0;bat<num_bat;bat++) 
for(int blk=0;blk<num_blk;blk++) 
  // Sender on the PL side
  // Buff Controller: SRAM Addr generation support
  //for data reuse and coarse-grained transpose
  buff_addr_gen(stream_addr0)      
  buff_load(buff_in,stream_addr0,stream_data0)
  axis_gen(stream_data0,stream_plio_lhs[0:3])
  axis_gen(..., stream_plio_rhs[0:7])

  // AIE Array Spatial Loop
  for(int m.0=0;m.0=A;m.0++)  
  for(int n.0=0;n.0=C;n.0++) 
  for(int k.0=0;k.0=B;k.0++)
    //Single AIE Time loop with 3D-SIMD Ins
    for(int m.1=0;m.1<I;m.1++)
    for(int n.1=0;n.1<J;n.1++)
    for(int k.1=0;k.1<K;k.1++)
       ...
       3D-SIMD(m.1,k.1,n.1); //128 MACs/cyc

  // Receiver on the PL side
  axis_receiver(stream_plio_out[0:1],stream_data1)
  softamx(stream_data1,stream_softmax)
  buff_addr_gen(stream_addr1)      
  buff_store(stream_addr1,stream_softmax,buff_out) 
\end{minted}
\label{code:Data flow}

% \end{minipage}
% \setlength{\textfloatsep}{0pt}% Remove \textfloatsep
% \setlength{\textfloatsep}{0pt}
\end{algorithm}
% \end{figure}[t]

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> Section4_Backup.tex <==
\subsection{SSR Hardware Design Methodology}
\label{sec:memory_allocation}
%In order to meet the stringent latency requirement in real-time decision-making scenarios, partitioning the large graphs into small sub-graphs and pinning the parameter into the on-chip buffer is well-adopted. 
In order to meet the stringent latency requirement in real-time decision-making scenarios, ~\M~ hugely reduces the off-chip memory access by pinning the weights in the on-chip buffer including the RAM on the PL side and the local memory of the AIE array side. Moreover, to further improve the overall latency, ~\M~ adopts the on-chip data forwarding to move the activations among multiple accelerators as well. However, memory allocation and on-chip data forwarding are non-trial in the system with high heterogeneity.

%there are two main challenges that need to be addressed so that it can make full use of the heterogeneous resources while avoiding the latency overhead among spatial accelerators.

\noindent\textbf{Memory allocation impacts not just the on-chip storage utilization but also plays a crucial role in determining the design strategy of the AIE array.} As demonstrated in CHARM~\cite{charmFPGA23} and AutoMM~\cite{AutoMM}, effective utilization of PLIOs is a fundamental aspect in sustaining the throughput of the AIE array. Allocating parameters to the local memory of AIEs aids in conserving PLIOs for the right-hand side (RHS) operands, thereby achieving high routability and AIE utilization. However, there are two challenges that must be overcome to make this approach successful. \textcircled{1} The attention layers in transformer models involve two activation operands, which complicates the implementation of the PLIO reduction strategy when mixed with other layers. To apply the weights pining and PLIO reduction strategy to the entire application graph, we mark each inter-layer assignment with an optimizable flag. This is achieved by checking if attention layers are included in this assignment. For example, the graph of one block of the transformer model is shown in Figure~\ref{fig:workload_partition}(a) where node 1 and 2 represents the attention layers with two activation inputs. When applying inter-layer partitioning strategy 1, only non-attention layers are assigned to accelerator 1, thus we enable the optimization for searching the configuration to pin all the weights in the local memory of AIEs.   \textcircled{2} However, an inadequate weight pinning strategy results in a decrease in computational efficiency for the VLIW-based vector AIE cores.  More specifically, the overall computation throughput is decided by both the number of parallel AIEs and the workload partitioned to a single AIE. As shown in Figure~\ref{fig:workload_partition}(b), workload 3 which assigns the whole workload to a single AIE doesn't work since it can't fit all the weights in the local memory. Compared to workload 2, workload 1 utilizes more AIEs but with lower single AIE efficiency. The trade-off becomes more obvious when scaling out to multiple accelerator resources and workload partitioning. Thus to hold the weights in the local memory of AIE while achieving high AIE efficiency, the workload of each AIE should be specialized during the design space exploration (DSE) stage. This approach differs from the strategy used in CHARM~\cite{charmFPGA23} and AutoMM~\cite{AutoMM} where the workload of a single AIE is fixed in the DSE.

%For example, a matrix multiply kernel with size 32$\times$192$\times$192 can be partitioned and pinned to 4*6 AIEs. Each AIE is capable of computing the workload with size 32$\times$48$\times$32 under 50\% efficiency.  

\begin{figure}[tb]
\centering
\includegraphics[width=1\columnwidth]{figures/force_partition.pdf}
\caption{On-chip data forwarding between spatial accelerators with force RAM bank partition.}
\vspace{5pt}
\label{fig:force_partition}
\end{figure}

\noindent\textbf{Different parallel strategies of spatial accelerators resulting in large latency overhead during on-chip forwarding.}
We illustrate the latency overhead by using a consecutive matrix multiply scenarios as shown in Figure~\ref{fig:force_partition}(a) where MatMul0 and MatMul1 are mapped to HMK0 and HMK1 respectively. The output matrix of Matmul0 will be forwarded as the input activation of Matmul1.  

When designing the spatial accelerators for MM with size M$\times$K$\times$N, there are three corresponding parallel choices at the AIE array level including here noted as A, B, and C. In the following case, while HMK0 parallels on A and C forming a 2$\times$2 AIE array, the HMK1 parallels on A and B forming a 4$\times$1 AIE array. To prevent the AIE array stream from stalling, A$\times$C tiles of output must be transferred through PLIO and received by the downstream PL BRAM/URAM simultaneously thus A$\times$C bank partitioning is required shown in the RAM of spatial accelerator0. However, the data stored in the 2$\times$2 banks needs to be forwarded to the subsequent spatial accelerators 1 as input activation in the format of 4$\times$1, resulting in bank conflicts. One straightforward solution to resolve bank conflicts is to introduce a non-overlapping operation that moves the data from RAM0 to RAM1 sequentially thus introducing a huge latency overhead in the pipeline as illustrated in Figure~\ref{fig:force_partition}(c). In this work, we propose a force-partition strategy to resolve the bank conflicts, while maintaining low latency. More specifically, we force the RAM bank partition of the subsequent HMK1 to be compatible with the previous HMK0 so that the on-chip forwarding latency can be overlapped by HMK0. In order to enable the force partition strategy, we take the on-chip forwarding overhead as a punishment during the design space exploration phase. So that it results in the proper parallel configuration among the spatial accelerators which extra bank partition can avoid the huge latency overhead.

% \subsection{Three-level Dataflow of A Single Spatial Accelerator}
% The key component of our proposed architecture is the spatial accelerators which comprise HMM and HCE units. We use spatial accelerator 4 which calculates $softmax(Q * K^T)$  as an example to illustrate the three-level dataflow of a single spatial accelerator. The pseudo-code is shown in Listing~\ref{code:Data flow}. 

% \noindent\textbf{Single AIE 3D-SIMD Instruction Level (Lines 16-21).}
% In the single AIE level, an MM with size $I * K * J$ is calculated by carefully packing the VLIW instructions and orchestrating the data movement between its local memory and registers.

% \noindent\textbf{AIE Array Parallel Execution Level (Lines 12-15).}
% In the AIE array level, the entire MM workload is distributed among multiple AIEs ($A * C * B$) for parallel computing. The temporal result is transferred to the neighboring AIE through the cascade stream in a fine-grained manner and finally sent to PL with the PLIO stream from the tail AIE in the chain.
% \input{Listing_Dataflow}
% \noindent\textbf{PL Kernel FIFO Stream Level (Lines 1-10 \& 23-27).}
% Given the flexibility from PL, the nonlinear and element-wise kernels such as Transpose and $softmax$ are mapped to the DSPs and LUTs on PL. 
% The kernels within each spatial accelerator are connected via the FIFO streams so that the data from the upper stream (AIE) can be directly processed by the PL kernels in the same pipeline manner with small or no runtime overhead. 
% Finally, all the intermediate activations are stored in the on-chip buffer managed by the buffer controllers and will be forwarded to the next spatial accelerator without any off-chip access.

% \subsection{~\M~ Hardware Design Methodology}
% \noindent\textbf{High Utilization Matrix Multiply Design on Single AIE and AIE Array.}
% % The hardware utilization is essential to the overall latency, especially in critical real-time scenarios. 
% % High computation capacity does not necessarily translate to high performance, especially in a task with inherently low parallelism, e.g., small batch inference. 
% % When designing the MM/BMM kernels under INT8 data type, efficient communication between PL SRAM, AIE local memory, and registers is important to saturate the high throughput. 
% % Thus we optimize MM/BMM kernels from two levels, i.e., the single AIE and AIE array level.
% Hardware utilization is essential in improving the overall performance, which is especially important in critical real-time cases. However, the high computation capacity of devices doesn't guarantee high performance of tasks, especially those with inherently low parallelism, e.g., small batch inference. To saturate the high throughput in likewise tasks, it's important to ensure efficient communication between PL SRAM, AIE local memory, and registers in MM/BMM kernels designation. To address this problem, we optimize these kernels from 2 levels: the single AIE and AIE array level.

% \begin{figure}[tb]
% \centering
% \includegraphics[width=1\columnwidth]{figures/single_aie_design.pdf}
% \vspace{-15pt}
% \caption{Efficient Single AIE Design.}
% \label{fig:single_AIE}
% \end{figure}

% In the single AIE level, based on the byte-level flexibility of AIE, we design customized instructions and make full use of the 2Kb vector register to sustain the 128 MACs/cycle throughput with two 256 bits/cycle load instructions. The 128 MACs can be constructed as a 16x8 MAC array as shown in Figure~\ref{fig:single_AIE} where the second dimension is the reduction dimension. 
% Under the constraints of 2Kb vector register as well as the 256 bits/cycle load bandwidth, we customize the 128 MACs into an 8*8*2 3D-SIMD instruction. 
% We allocate 8*8 and 8*4 8bits vector registers and use the double buffer technique to hide the latency of loading from local memory to the vector registers. 
% When launching 8*8*2 3D-SIMD in two cycles, we can load another 8*8 and 8*4 INT8 registers at the same time.

% At the single AIE level, we design customized instructions to saturate 128 MACs/cycle throughput under the constraints of the 2Kb vector register and the 256 bits/cycle load bandwidth. As shown in  Figure~\ref{fig:single_AIE}, the 128 MACs and be constructed as a 16x8 MAC array in which the reduced dimension acts as the second dimension. To sustain the throughput, we customize the MACs into an 8*8*2 3D-SIMD instruction and use the double-buffer technique to overlap the latency of loading and storing data: we allocate 2 groups of 8*8 and 8*4 8 bits vector registers, on the one hand, launching the SIMD instructions will take 2 cycles to finish computation for one group, on the other hand, the other group of register can be also loaded in 2 cycles also in 2 cycles.  

% When scaling out to the AIE array, only 156 PLIOs(128bits each) are available to sustain the throughput of 400 AIEs. 
% To better optimize the data communication between AIE and PL, we propose two kinds of HMM units as shown in Figure~\ref{fig:proposed_arch}. HMM Units 0 and 4 form two $1* 2 * 4$ spatial systolic arrays corresponding to the $A * C * B$ spatial loop demonstrated in Listing~\ref{code:Data flow}. 
% Both of them explore the broadcast opportunity to reuse the PLIO as illustrated by the left-hand-side (LHS) PLIO which reduces the demand for PLIOs from 8 to 4. 
% For the first type of AIEs that take both the activation and weights as their operands, we efficiently allocate the AIE local memory to make sure the weight of all the blocks fit and loaded during initialization without further excessive loads.
% Thus it saves the PLIO of sending the right-hand-side (RHS) operands (weights). 
% However, for the kernels that the weights can't fit in the AIE local memory or the two operands are both activations (attention batch dot), we map them to the second type of AIE design. 
% Comparing HMM Unit0 to HMM Unit4 that utilizes 2x4 AIEs, HMM Unit0 saves 8 PLIOs on the right-hand-side(RHS) operands and this  results in a high utilization as 98.5\% of the total 400 AIEs. 

==> tables/prior_compare_old.tex <==

\begin{table*}
    \centering
\caption{\textcolor{black}{Comparisons with prior works.}}
% \vspace{-5pt}
\footnotesize
\begin{adjustbox}{width=2\columnwidth,center}
\begin{tabular}{c|cc|cccccc}
\toprule
\multirow{2}{*}{\makecell[cc]{\textbf{Prior Works}}}  & \multicolumn{2}{c|}{\makecell[cc]{\textbf{Computing} \textbf{Platform}} }    &\multicolumn{6}{c}{\textbf{Architecture Features}}  \\ 
\cline{2-9}
  &\textbf{Board Type} & \textbf{GOPS/(GB/s)}   & \makecell[cc]{\textbf{Spatial}\\\textbf{Accelerator}} &  \makecell[cc]{\textbf{Hardware}\\\textbf{Specialization}} &  \makecell[cc]{\textbf{On-chip}\\\textbf{Forwarding}}  & \makecell[cc]{\textbf{Fine-grained }\\\textbf{Pipeline}}& \makecell[cc]{\textbf{Hybrid}} & \makecell[cc]{\textbf{Layout}\\\textbf{Change}} \\
\midrule

\makecell[cc]{{TensorRT}~\cite{vanholder2016efficientTensorRT}} &\textcolor{black}{GPU} & {\textcolor{black}{--}} &\textcolor{red}{$\times$} &\textcolor{red}{$\times$} &\textcolor{red}{$\times$}&\textcolor{red}{$\times$} &\textcolor{red}{$\times$} &\textcolor{red}{$\times$}  \\
\arrayrulecolor{black!30}\midrule

% \makecell[cc]{{\color{violet}Herald}~\cite{kwon2021heterogeneous}} &ASIC&\textcolor{black}{--} &\textcolor{ForestGreen}{\checkmark}&\textcolor{red}{$\times$}  &\textcolor{red}{$\times$} &\textcolor{red}{$\times$}&\textcolor{black}{--} &{High}    \\
% \midrule

\makecell[cc]{{MAGMA}~\cite{kao2022magma}, {Herald}~\cite{kwon2021heterogeneous}} &ASIC &\textcolor{black}{--}&\textcolor{ForestGreen}{\checkmark} & \textcolor{ForestGreen}{\checkmark} & \textcolor{red}{$\times$} &\textcolor{red}{$\times$}&\textcolor{ForestGreen}{\checkmark}&\textcolor{red}{$\times$}     \\
\midrule

% \makecell[cc]{{\color{violet}ViA}~\cite{wang2022via}} &{FPGA U50} &{372/316=1.18}&\textcolor{ForestGreen}{\checkmark} &\textcolor{ForestGreen}{\checkmark}&\textcolor{red}{$\times$}&\textcolor{ForestGreen}{\checkmark}&\textcolor{red}{$\times$} &{High}   \\
% \midrule


\makecell[cc]{{CHARM}~\cite{charmFPGA23}} &{ACAP VCK190} &{6400/25.6=250}& \textcolor{ForestGreen}{\checkmark} & \textcolor{ForestGreen}{\checkmark}  &\textcolor{red}{$\times$} &\textcolor{ForestGreen}{\checkmark} &\textcolor{ForestGreen}{\checkmark}&\textcolor{red}{$\times$}   \\
\midrule

\makecell[cc]{{ViTCoD}~\cite{you2023vitcod}} &{ASIC} &{256/76.8=3.3}&\textcolor{red}{$\times$}&\textcolor{ForestGreen}{\checkmark}&\textcolor{red}{$\times$}&\textcolor{red}{$\times$}&\textcolor{red}{$\times$} &\textcolor{red}{$\times$}   \\
\midrule

\makecell[cc]{{HeatViT}~\cite{dong2023heatvit}, Auto-ViT-Acc}~\cite{lit2022auto} &{FPGA ZCU102} &{1260/19.2=65.6}&\textcolor{red}{$\times$}&\textcolor{ForestGreen}{\checkmark} &\textcolor{red}{$\times$}&\textcolor{red}{$\times$}&\textcolor{red}{$\times$} &\textcolor{red}{$\times$}  \\
\midrule



\makecell[cc]{{BrainWave}~\cite{putnam2014reconfigurable,caulfield2016cloud,firestone2018azure,fowers2018configurable,boutros2020beyond}, Intel NPU~\cite{boutros2020beyond}} &{FPGA Stratix 10} &{143000 /512=279.3}&\textcolor{ForestGreen}{\checkmark}&\textcolor{ForestGreen}{\checkmark}&\textcolor{ForestGreen}{\checkmark}&\textcolor{red}{$\times$}&\textcolor{red}{$\times$} &\textcolor{red}{$\times$}  \\
\midrule

% \makecell[cc]{~\cite{boutros2020beyond}} &{FPGA Stratix 10 NX} &{}&\textcolor{ForestGreen}{\checkmark}&\textcolor{ForestGreen}{\checkmark}&\textcolor{ForestGreen}{\checkmark}&\textcolor{red}{$\times$}&\textcolor{red}{$\times$} & {\bcancel{\checkmark}}  \\
% \midrule

% \makecell[cc]{{\color{teal}DNNBuilder}~\cite{zhang2018dnnbuilder}} &{FPGA XC7Z045 and
% KU115} &{-}&\textcolor{ForestGreen}{\checkmark}&\textcolor{ForestGreen}{\checkmark}&\textcolor{ForestGreen}{\checkmark}&\textcolor{red}{$\times$}&\textcolor{red}{$\times$} &\textcolor{red}{$\times$}   \\
% \midrule

\makecell[cc]{{DNNExplorer}~\cite{zhang2020dnnexplorer}} &{FPGA 
KU115} &{-}&\textcolor{ForestGreen}{\checkmark}&\textcolor{ForestGreen}{\checkmark}&\textcolor{ForestGreen}{\checkmark}&\textcolor{red}{$\times$}&\textcolor{ForestGreen}{\checkmark} &\textcolor{red}{$\times$}   \\
\midrule

\makecell[cc]{{SET}~\cite{MaKaishengISCA23}} &{ASIC} &{-}&\textcolor{ForestGreen}{\checkmark}&\textcolor{ForestGreen}{\checkmark}&\textcolor{ForestGreen}{\checkmark}&\textcolor{red}{$\times$} &\textcolor{ForestGreen}{\checkmark}&\textcolor{red}{$\times$}    \\
\midrule

\makecell[cc]{{DiviML}~\cite{ghannane2023diviml}} &{CPU+GPUs} &{-}&\textcolor{ForestGreen}{\checkmark}&\textcolor{ForestGreen}{\checkmark}&\textcolor{red}{$\times$}&\textcolor{red}{$\times$}&\textcolor{ForestGreen}{\checkmark} &\textcolor{red}{$\times$}   \\

% \makecell[cc]{{\color{teal}Auto-ViT-Acc}~\cite{lit2022auto}} &{FPGA ZCU102} &{1260/19.2=65.6}&\textcolor{red}{$\times$}&\textcolor{ForestGreen}{\checkmark} &\textcolor{red}{$\times$}&\textcolor{red}{$\times$}&\textcolor{ForestGreen}{\checkmark} &{High} \\
%\midrule


\arrayrulecolor{black}\specialrule{0.75pt}{1pt}{3pt}

\makecell[cc]{\textbf{{SSR}}\\\textbf{(Ours)}} &{ACAP VCK190}&{102,400/25.6=4000}    &\textcolor{ForestGreen}{\checkmark}&\textcolor{ForestGreen}{\checkmark}&\textcolor{ForestGreen}{\checkmark}&\textcolor{ForestGreen}{\checkmark}&\textcolor{ForestGreen}{\checkmark}&\textcolor{ForestGreen}{\checkmark} \\
\arrayrulecolor{black}\specialrule{0.75pt}{1pt}{3pt}

%\bottomrule
\end{tabular}
\end{adjustbox}
\label{Prior_Comparison}
  % {\raggedright \scriptsize Note: 
  % {  %\color{violet}Purple} indicates architecture and mapping framework. 
  % ~\cite{vanholder2016efficientTensorRT,kwon2021heterogeneous,kao2022magma,wang2022via,charm2023} are \textcolor{violet}{architecture and mapping frameworks}. 
  % %{\color{teal} Green} 
  % ~\cite{lit2022auto,dong2023heatvit,you2023vitcod} and \M~(ours) are \textcolor{teal}{algorithm-hardware co-design frameworks}.
  % \par}
  % }
  % \vspace{-20pt}
\end{table*}

==> zz.tex <==
\author{Jinming Zhuang}
\email{jinming.zhuang@pitt.edu}
\orcid{0000-0003-3659-339X}
\affiliation{%
  \institution{University of Pittsburgh}
  \streetaddress{3700 O’Hara Street}
  \city{Pittsburgh}
  \state{Pennsylvania}
  \country{USA}
  \postcode{15261}}

\author{Zhuoping Yang}
\orcid{0000-0002-7655-4080}
\email{zhuoping.yang@pitt.edu}
\affiliation{%
  \institution{University of Pittsburgh}
  \streetaddress{3700 O’Hara Street}
  \city{Pittsburgh}
  \state{Pennsylvania}
  \country{USA}
  \postcode{15261}}


\author{Shixin Ji}
\email{shixin.ji@pitt.edu}
\orcid{0009-0003-3429-4692}
\affiliation{%
  \institution{University of Pittsburgh}
  \streetaddress{3700 O’Hara Street}
  \city{Pittsburgh}
  \state{Pennsylvania}
  \country{USA}
  \postcode{15261}}

\author{Heng Huang}
\email{heng@umd.edu}
\affiliation{%
  \institution{University Maryland College Park}
  \city{College Park}
  \state{Maryland}
  \country{USA}
  \postcode{20742}}

\author{Alex Jones}
\email{akjones@pitt.edu}
\orcid{0000-0001-7498-0206}
\affiliation{%
  \institution{University of Pittsburgh}
  \streetaddress{3700 O’Hara Street}
  \city{Pittsburgh}
  \state{Pennsylvania}
  \country{USA}
  \postcode{15261}}

\author{Jingtong Hu}
\email{jthu@pitt.edu}
\orcid{0000-0003-4029-4034}
\affiliation{%
  \institution{University of Pittsburgh}
  \streetaddress{3700 O’Hara Street}
  \city{Pittsburgh}
  \state{Pennsylvania}
  \country{USA}
  \postcode{15261}}

\author{Yiyu Shi}
\email{yshi4@nd.edu}
\orcid{0000-0002-6788-9823}
\affiliation{%
  \institution{University of Notre Dame}
  \streetaddress{325D Cushing Hall of Engineering}
  \city{Notre Dame}
  \state{Indiana}
  \country{USA}
  \postcode{46556}}

\author{Peipei Zhou}
\orcid{0000-0002-0493-1844}
\affiliation{%
  \institution{University of Pittsburgh}
  \streetaddress{3700 O’Hara Street}
  \city{Pittsburgh}
  \state{Pennsylvania}
  \country{USA}
  \postcode{15261}}
\email{peipei.zhou@pitt.edu}

%%
%% By default, the full list of authors will be used in the page
%% headers. Often, this list is too long, and will overlap
%% other information printed in the page headers. This command allows
%% the author to define a more concise list
%% of authors' names for this purpose.
\renewcommand{\shortauthors}{Jinming Zhuang et al.}
